The importance of being constrained: dealing with infeasible solutions in Differential Evolution and beyond

We argue that results produced by a heuristic optimisation algorithm cannot be considered reproducible unless the algorithm fully specifies what should be done with solutions generated outside the domain, even in the case of simple box constraints. Currently, in the field of heuristic optimisation, such specification is rarely mentioned or investigated due to the assumed triviality or insignificance of this question. Here, we demonstrate that, at least in algorithms based on Differential Evolution, this choice induces notably different behaviours - in terms of performance, disruptiveness and population diversity. This is shown theoretically (where possible) for standard Differential Evolution in the absence of selection pressure and experimentally for the standard and state-of-the-art Differential Evolution variants on special test function $f_0$ and BBOB benchmarking suite, respectively. Moreover, we demonstrate that the importance of this choice quickly grows with problem's dimensionality. Different Evolution is not at all special in this regard - there is no reason to presume that other heuristic optimisers are not equally affected by the aforementioned algorithmic choice. Thus, we urge the field of heuristic optimisation to formalise and adopt the idea of a new algorithmic component in heuristic optimisers, which we call here a strategy of dealing with infeasible solutions. This component needs to be consistently (a) specified in algorithmic descriptions to guarantee reproducibility of results, (b) studied to better understand its impact on algorithm's performance in a wider sense and (c) included in the (automatic) algorithmic design. All of these should be done even for problems with box constraints.

==> proofs.tex <==
Anna moved it to the end of main paper

==> tableSDIS_copy.tex <==
\begin{landscape}
\centering
% \begin{adjustbox}{width=1.3\textwidth}
\begin{threeparttable}%[!tb]
{\small
\caption{\hl{to move, re-number footnotes} Previous studies on the influence of SDIS on DE, with dictionary for SDIS alternative terminology\label{tab:PreviousStudied}}
%\begin{tabular}{|p{0.085\linewidth}|p{0.13\linewidth}|p{0.13\linewidth}|p{0.13\linewidth}|p{0.13\linewidth}|p{0.13\linewidth}|p{0.13\linewidth}|}
\begin{tabular}{p{0.085\linewidth}p{0.13\linewidth}p{0.13\linewidth}p{0.145\linewidth}p{0.15\linewidth}p{0.11\linewidth}p{0.13\linewidth}}
\toprule
\textbf{Paper} & \cite{Arabas2010} & \cite{Padhye2015} & \cite{Kreischer2017} & \cite{bib:BIEDRZYCKI2019} & \cite{Boks2021}& This paper \\ 
\midrule
\textbf{Benchmark} & CEC 2005 & 4 functions\footnotemark & CEC 2017 & CEC 2017 & BBOB & BBOB \\ 
\midrule
% DE variants, parameter settings & DE/rand/1/bin, $C_r=0.9$, $F=0.8$ & DE/best/1/bin, $C_r=0.5$, $F=0.7$ – for $n=20$, $C_r=0.9$, $F=0.8$ for $n=$\hl{?} & DE/target-to-best/1/bin, $C_r=0.9$, $F=0.8$ & DE/rand/1/bin, $C_r=1$, $F=0.9$, DE/local-to-best/1/bin, SADE, JADE, jSO, DES, BBDE & SHADE \hl{?} & DE/rand/1/bin, $25-50$ values of $F$ and $C_r$, SHADE, L-SHADE\\ 
\textbf{Standard DE variants, $(F,C_r)$} & DE/rand/1/bin,  $(0.8,0.9)$ & DE/best/1/bin, $(0.7,0.5), (0.8,0.9)$\footnotemark & DE/target-to-best/1/bin, $(0.8,0.9)$ & DE/rand/1/bin, $(0.9,1)$, DE/local-to-best/1/bin & 15 mutation $\times$ 2 crossover ope\-ra\-tors, SHADE adaptation & DE/rand/1/ with 2 crossovers, 25-50 uniformly spaced $(F,C_r)$ values\\ 
\midrule
\textbf{Advanced DE variants} & -- & -- & -- & SADE, JADE, jSO, DES, BBDE & -- & SHADE, L-SHADE\\ %hyper adaptive SHADE
\midrule
\textbf{Coordinate-} & reflection & -- & reflection & reflection & reflection & mirror \\ 
\cmidrule{2-7}
\textbf{wise SDIS} & projection & set on boundary & projection & projection & projection & saturation \\ 
\cmidrule{2-7}
& wrapping & periodic & -- & wrapping & wrapping & toroidal \\ 
\cmidrule{2-7}
& reini\-tia\-lisation & random & reini\-tia\-lisation & reini\-tia\-lisation & reini\-tia\-lisation & uniform \\ 
\cmidrule{2-7}
& -- & -- & -- & midpoint to target & midpoint target & halfway \\ 
\cmidrule{2-7}
& -- & -- & midpoint to base & midpoint to base & midpoint base & -- \\ 
\cmidrule{2-7}
& -- & expo\-nen\-tia\-lly confined, spread & -- & -- & -- & COTN \\ 
\cmidrule{2-7}
& -- & -- & -- & -- & other SDIS\footnotemark & -- \\ 
\midrule
\textbf{Vector-wise SDIS} & -- & shrink\footnotemark & scaled mutant\footnotemark & projection to midpoint or base\footnotemark & -- & -- \\ 
\cmidrule{2-7}
& -- & inverse parabolic (confined, spread) & -- & -- & -- & -- \\ 
\bottomrule
\end{tabular}
\begin{tablenotes}
\item[4] Unimodal test functions (Ellipsoidal, Schwefel, Ackley, Rosenbrock)
\item[5] For $n=20$ and $n\in\{50, 100, 200, 300, 500\}$, respectively
\item[6] Death-penalty, resampling, boundary-transformation, rand-base, projection-to-midpoint, projection-to-base
\item[7] Linear combination between the trial and base elements
\item[8] Linear combination between the trial and a reference elements in the feasible region
\item[9] Linear combination between the trial and the domain midpoint or base element
\end{tablenotes}
}
\end{threeparttable}
% \end{adjustbox}
\end{landscape}

==> viridis_def.tex <==
%https://bookdown.org/hneth/ds4psy/D-2-apx-colors-essentials.html
\definecolor{viridis_1_10}{RGB}{68,1,84}
\definecolor{viridis_2_10}{RGB}{72,40,120}
\definecolor{viridis_3_10}{RGB}{62,74,137}
\definecolor{viridis_4_10}{RGB}{49,104,142}
\definecolor{viridis_5_10}{RGB}{38,130,142}
\definecolor{viridis_6_10}{RGB}{31,158,137}
\definecolor{viridis_7_10}{RGB}{53,183,121}
\definecolor{viridis_8_10}{RGB}{109,205,89}
\definecolor{viridis_9_10}{RGB}{180,222,44}
\definecolor{viridis_10_10}{RGB}{253,231,37}
%
%colours used in EDPOIS plots
\definecolor{POIS_teal}{RGB}{99,172,190} % #63ACBE 
\definecolor{POIS_orange}{RGB}{238,68,47} % #EE442F, 99.9-100%
\definecolor{POIS_violet}{RGB}{96,26,47} % #601A4A 1-99%, 99-99.9%
